Cancellation-Free Constrained SquareCB for Safe Controller Selection

We study constrained contextual bandits, in which a learner chooses one of $K$ actions in each round to minimize loss while keeping the expected cost of its play below a budget. Existing reductions to online regression weight the cost by a Lagrange multiplier learned from past constraint residuals, so slack in some rounds can offset violations in others. We instead run SquareCB proposed in \citep{foster2020beyond} with a rectified weight on the cost: it is zero when the estimated cost is within the budget, and otherwise just large enough to bring it back to the budget. Under realizability and Slater's condition with margin $\delta$, the algorithm attains regret $O(\sqrt{KT\,\mathrm{Reg}_{\mathsf{Sq}}(T)}/\delta)$ and cancellation-free violation $\sum_t(V_c^{p_t}-b)^+=O(\sqrt{KT\,\mathrm{Reg}_{\mathsf{Sq}}(T)})$, where $\mathrm{Reg}_{\mathsf{Sq}}$ is the error of the regression oracle. The same bounds hold when the budget must be met in every context, potentially adversarially chosen contexts. In controller selection for a safe-control-gym quadrotor and a BOPTEST building, the violation is 6 to 9 times lower than that of primal-dual and virtual-queue baselines, with a lower or comparable regret.

==> introduction.tex <==
Contextual Bandits (CBs) are an online learning framework widely used for sequential decision-making under uncertainty. They can be viewed as a generalization of the Multi-Armed Bandit (MAB) problem, in which the learner's action-selection strategy is conditioned on an observed input vector, commonly referred to as the context. In contrast, in the classical MAB setting, action selection is independent of any contextual information.

CBs have found applications in a wide range of domains, including personalized recommendation systems \citep{li2010contextual, feijer2025calibrated}, crowdsourcing \citep{muller2018context, elahi2023online}, and medical studies \citep{tewari2017ads, huch2024rome}. Formally, a CB problem involves sequential interaction between a learner and an environment. At each round, the learner observes a context, selects an action based on the observed context, and subsequently receives feedback in the form of a reward associated with the chosen action \citep{langford2007epoch, lattimore2020bandit}. The learner uses this feedback to improve its future decisions. The CB framework has been extensively studied, with a rich body of literature addressing both unconstrained and constrained settings and providing algorithms with provable performance guarantees and near-optimal regret bounds.

Despite their widespread applicability, many real-world decision-making problems cannot be adequately modeled using the standard unconstrained CB framework \citep{badanidiyuru2018bandits, badanidiyuru2014resourceful, agrawal2016linear}. In practice, maximizing the expected reward is often insufficient, as the learner must simultaneously satisfy additional operational requirements. These requirements naturally arise in the form of constraints that cannot be inherently captured by the vanilla CB objective. For instance, online recommendation and advertising platforms must optimize user engagement or advertisement placements while adhering to advertisers' budget constraints. In crowdsourcing applications, task allocation must account for fairness considerations and compliance with labor regulations. Similarly, in clinical trials, treatment allocation must balance patient-specific outcomes against limited medical resources and treatment-related safety requirements. Such applications require incorporating additional constraint functions alongside the reward objective, motivating the study of constrained rather than vanilla contextual bandits \citep{han2023optimal}.

To address these requirements, Constrained Contextual Bandits (CCBs) have been introduced and studied in several works \citep{wu2015algorithms, agrawal2016efficient}. The framework has recently received increasing attention due to its applicability to resource-constrained sequential decision-making problems \citep{slivkins2023contextual, guo2024stochastic, sarkar2026simple}. Unlike the vanilla CB setting, the objective in CCBs is to maximize the cumulative expected reward while simultaneously ensuring that the learner satisfies a prescribed long-run constraint on the cumulative expected cost (see Equation~\eqref{eqn}). Thus, the learner must balance reward maximization with constraint satisfaction throughout its interaction with the environment.

A fundamental challenge in contextual bandit learning is the development of general-purpose algorithms that can accommodate a broad class of user-specified policy classes while retaining strong theoretical guarantees. Such algorithms are particularly desirable because they allow practitioners to adapt the learning framework to different applications without having to design a new algorithm for every problem instance. In this direction, \citet{foster2020beyond} introduced an oracle-based framework for contextual bandits that accommodates general policy classes through computationally tractable optimization oracles, under suitable assumptions on the hypothesis class and the availability of efficient oracle implementations. This approach provides a flexible algorithmic framework without requiring restrictive structural assumptions on the underlying policy class.

Despite these advances in general-purpose contextual bandit algorithms, the constrained setting remains relatively under-explored. Although several works have investigated constrained contextual bandits (CCBs) ( \textcolor{red}{insert relevant references}), existing approaches leave room for improvement in the strength of their theoretical regret and constraint violation guarantees. In particular, conventional guarantees based on cumulative signed constraint violations may conceal substantial violations at individual rounds, as positive violations can be offset by negative constraint residuals in other rounds. Consequently, controlling the cumulative signed violation does not necessarily ensure that the learner consistently respects the prescribed constraint.

In this work, we address this limitation by considering a stronger notion of performance guarantees, which we refer to as cancellation-free regret and cancellation-free constraint violation. Unlike conventional guarantees that permit positive and negative terms to cancel each other, our formulation explicitly accounts for positive regret and constraint violations without allowing such cancellation. We propose an efficient algorithm that achieves improved cancellation-free regret and violation guarantees compared with existing online regression-based approaches ( \textcolor{red}{insert Rohan Deb's paper and other relevant CCB references}), under the Slater's condition assumption alone. This is particularly appealing because Slater's condition is a standard regularity assumption in constrained optimization and has also been adopted in several existing works on constrained contextual bandits ( \textcolor{red}{insert relevant references}). Our results therefore establish stronger performance guarantees under a commonly used feasibility assumption, without requiring additional restrictive assumptions.

\paragraph{Why is cancellation-free constraint violation challenging?}

The difficulty of obtaining cancellation-free guarantees can be understood through the standard Lagrangian reduction for constrained optimization. Such approaches typically maintain an adaptive Lagrange multiplier $\lambda_t$ that is updated using the signed constraint residual $V_c^{p_t}-b$. In particular, when the learner under-utilizes the available budget, i.e., $V_c^{p_t}<b$, the corresponding gradient is negative, causing the multiplier to decrease. Consequently, the learner can accumulate constraint slack during rounds in which the constraint is easily satisfied, allowing the multiplier to decrease toward zero. This, in turn, can permit substantial constraint violations in subsequent rounds before the multiplier increases sufficiently to penalize them.

More fundamentally, such an update mechanism controls the cumulative signed constraint residual,
\[
\sum_{t=1}^{T}(V_c^{p_t}-b),
\]
which allows positive and negative residuals to cancel each other. However, a small signed cumulative residual does not necessarily imply a small cumulative positive violation. For instance, consider the sequence of constraint residuals
\[
V_c^{p_t}-b =
\begin{cases}
+1, & t \text{ odd},\\
-1, & t \text{ even}.
\end{cases}
\]
For this sequence, the cumulative signed residual is at most one, whereas the cumulative positive violation is
\[
\sum_{t=1}^{T}(V_c^{p_t}-b)^+
=\left\lceil \frac{T}{2}\right\rceil,
\]
which grows linearly with the horizon. Thus, a guarantee on cumulative signed constraint violation alone is insufficient to establish a sublinear bound on cancellation-free violation. This illustrates the fundamental difficulty of obtaining stronger constraint satisfaction guarantees and motivates the development of algorithms that explicitly control positive violations without relying on the cancellation of constraint slack.

==> related_work.tex <==
Contextual bandits have been extensively studied under various problem settings, evolving from classical multi-armed bandits to more general nonlinear formulations. Early developments in multi-armed bandits established the foundations of sequential decision-making under uncertainty, with several influential works providing regret guarantees for learning to select among a finite set of actions \textcolor{red}{(Auer et al., 2002; Agarwal and Goyal, 2012; Bubeck et al., 2012; Bubeck and Slivkins, 2012)}. However, the absence of contextual information in the classical multi-armed bandit formulation limits its ability to capture decision-making problems where the optimal action depends on the characteristics of the environment or the user. This limitation becomes particularly relevant in applications such as personalized recommendation systems, where decisions must adapt to high-dimensional and potentially heterogeneous user contexts. Consequently, contextual bandits with linear function representations received considerable attention, with several works establishing strong theoretical guarantees for linear reward and cost functions \textcolor{red}{(Chu et al., 2011; Abbasi-Yadkori et al., 2011; Agrawal and Goyal, 2013)}. Linear contextual bandits have since become an important framework for applications requiring efficient learning and generalization from contextual information \textcolor{red}{(cite applications)}.

Despite their theoretical tractability, linear representations can be restrictive when the underlying reward or cost functions exhibit complex nonlinear dependencies on the contexts and actions. This motivated the development of nonlinear contextual bandit algorithms, particularly those based on neural networks. A series of works on neural contextual bandits \textcolor{red}{(Zahavy and Mannor, 2020; Zhou et al., 2020; Zhang et al., 2021)} introduced algorithms capable of handling general nonlinear function representations and established corresponding regret guarantees, thereby expanding the applicability of contextual bandits to more complex real-world problems. Nevertheless, designing and analyzing such algorithms often requires additional structural assumptions and problem-specific modifications, which can limit their applicability across different function classes and learning tasks.

An alternative approach to handling general function representations is to reduce contextual bandit learning to online regression. In particular, \textcolor{red}{(cite(Foster and Rakhlin 2020 and Foster and Krisnmurthy 2021)} developed general reduction frameworks based on the Inverse Gap Weighting (IGW) principle \textcolor{red}{(Abe and Long, 1999; Abe et al., 2003)}. These reductions decouple the exploration strategy from the choice of function approximator by relying on an online regression oracle, allowing the resulting regret guarantees to be expressed in terms of the regression oracle's performance. This provides a flexible framework for contextual bandits beyond conventional linear representations. Building on this direction, \textcolor{red}{(cite Deb et al. (2025))} studied conservative contextual bandits beyond linear representations and proposed \emph{C-SquareCB} and \emph{C-FastCB}, which employ squared-loss and KL-loss regression oracles, respectively. By instantiating these oracles with neural networks and online gradient descent, they obtained regret guarantees of $\widetilde{O}(\sqrt{KT}+K/\alpha)$ and $\widetilde{O}(\sqrt{KL^{*}}+K(1+1/\alpha))$, respectively, where $T$ denotes the horizon and $L^{*}$ denotes the cumulative loss of the optimal policy. Their work demonstrates the effectiveness of regression-oracle-based reductions in extending contextual bandit algorithms to nonlinear settings while maintaining conservative performance guarantees.

While these developments have significantly advanced contextual bandit learning, incorporating explicit constraints on the learner's decisions introduces additional challenges. In particular, conservative contextual bandits, such as those studied by \textcolor{red}{(Deb et al. (2025))}, impose performance guarantees relative to a baseline policy, whereas constrained contextual bandits require the learner to optimize an objective subject to an explicit cost budget. These formulations lead to different notions of feasibility and require different algorithmic and analytical considerations.

Several works have investigated constrained contextual bandits using regression-oracle-based approaches. \citep{slivkins2023contextual} extended the SquareCB framework to contextual bandits with packing and covering constraints through a modular Lagrangian approach, in which the constraint costs are incorporated into the objective using dual variables updated via online learning. More recently, \citep{sarkar2026simple} developed a reduction for constrained contextual bandits with adversarial contexts, replacing the Lagrange multiplier update with a virtual queue and a Lyapunov-based analysis. In both approaches, the cost weight is driven by the signed constraint residual, resulting in guarantees that control the cumulative signed constraint violation. However, such guarantees permit cancellation between rounds with positive and negative constraint residuals, potentially concealing repeated budget violations.

A natural approach to obtaining a one-sided guarantee is to apply these methods to the clipped constraint cost $(c-b)^+$. However, this controls $\sum_{t=1}^{T}\mathbb{E}_{a\sim p_t}[(c(a)-b)^+]$, which penalizes individual actions exceeding the budget, even when the expected cost under the played distribution satisfies the constraint. Consequently, this approach does not preserve the flexibility of randomized policies that combine actions with costs both above and below the budget, as may be required by the constrained optimum $\pi^*$. This can lead to overly conservative policies.

The distinction between signed and one-sided constraint guarantees has also been investigated in other sequential decision-making settings. In particular, \citep{efroni2020exploration} highlighted that conventional Lagrangian approaches for constrained Markov decision processes control cumulative signed constraint violations, allowing cancellation across time, whereas controlling the sum of positive constraint violations provides a stronger guarantee. Similarly, in online convex optimization with adversarial constraints, recent works have studied guarantees on the cumulative positive part of constraint residuals \citep{guo2022online,sinha2024optimal}. Motivated by these developments, we study cancellation-free constraint violation in contextual bandits through a regression-oracle-based reduction. Specifically, we retain the SquareCB framework and introduce a rectified cost weight, computed through bisection, to control the constraint violation without relying on a dual-ascent update. Combined with an exact-penalty saddle analysis, this yields cancellation-free violation and regret guarantees while preserving the flexibility of randomized policies.
